Visual Word2Vec (vis-w2v): Learning Visually Grounded Word Embeddings Using Abstract Scenes

We propose a model to learn visually grounded word embeddings (vis-w2v) to capture visual notions of semantic relatedness. While word embeddings trained using text have been extremely successful, they cannot uncover notions of semantic relatedness implicit in our visual world. For instance, although "eats" and "stares at" seem unrelated in text, they share semantics visually. When people are eating something, they also tend to stare at the food. Grounding diverse relations like "eats" and "stares at" into vision remains challenging, despite recent progress in vision. We note that the visual grounding of words depends on semantics, and not the literal pixels. We thus use abstract scenes created from clipart to provide the visual grounding. We find that the embeddings we learn capture fine-grained, visually grounded notions of semantic relatedness. We show improvements over text-only word embeddings (word2vec) on three tasks: common-sense assertion classification, visual paraphrasing and text-based image retrieval. Our code and datasets are available online.

==> approach/approach-points.tex <==
\begin{itemize}
	\item Intro that we describe how visual word2vec is trained in general and will explain nuances for each tasks at the end.
% * <vrama91@vt.edu> 2015-10-21T09:12:55.349Z:
%
% > \item Intro that we describe how visual word2vec is trained in general and will explain nuances for each tasks at the end.
%
% remove
%
% ^ <satwik27@gmail.com> 2015-10-21T14:50:58.824Z:
%
% So we only talk about how vis-w2v is trained generally ? 
%
% ^.
    \item Ingredients - pre-trained word2vec model, multi-modal data represented by visual features and associated text.
    \item overall procedure : take the word2vec model, cluster the visual features to get surrogate labels. Refine the network by predicting these labels with the help of associated text.
% * <vrama91@vt.edu> 2015-10-21T09:13:32.414Z:
%
% >  \item Ingredients - pre-trained word2vec model, multi-modal data represented by visual features and associated text.
%
% Since we try different corpora for training word2vec, talk of it as if it is also a part of your approach. We train word2vec on blah.. instead of saying we take pretrained w2v
%
% ^ <satwik27@gmail.com> 2015-10-21T14:51:09.824Z:
%
% Alright.
%
% ^.
    \item Thus we train the visualword2vec embeddings.
    \item We will describe each part in detail.
% * <vrama91@vt.edu> 2015-10-21T09:14:19.114Z:
%
% > We
%
% Sounds good
%
\end{itemize}

\subsection{Clustering of Images}
% Argue regression on features might overfit
\begin{itemize}
	\item neural networks need supervised data to train
% * <vrama91@vt.edu> 2015-10-21T09:14:58.104Z:
%
% > 	\item neural networks need supervised data to train
%
% Unnecessary to say this. Deep Belief Nets, RBM's etc are a whole class of NN which are trained without supervision
%
	\item Therefore, we cluster the visual features of the train dataset as a first step to get surrogate labels.
	\item visual word2vec is then trained by predicting these labels using the associated text as the input.
    \item We found this strategy to perform better than regressing on the features
% * <vrama91@vt.edu> 2015-10-21T09:15:50.907Z:
%
% > We found this strategy to perform better than regressing on the features
%
% We should invesitgate this further. Is this only because the regression problem is difficult or because clustering is somehow the right thing to do? What is the preformance of this regression model, btw? We will report this in the results right?
%
% ^ <satwik27@gmail.com> 2015-10-21T14:52:02.722Z:
%
% I haven't tried with the regression model. This task was deferred. Perhaps, now is the time to get it done.
%
% ^.
    \item This could be due to the fact that visual features capture rich semantic features like orientation, size, flip, depth etc., and are of high dimensional. Regression can outfits given the small size of the multi-modal training data. \satwik{can we claims something like this?}
% * <vrama91@vt.edu> 2015-10-21T09:17:35.799Z:
%
% >  This could be due to the fact that visual features capture rich semantic features like orientation, size, flip, depth etc., and are of high dimensional. Regression can outfits given the small size of the multi-modal training data. \satwik{can we claims something like this?}
%
% We could drop this and just say that we wanted to capture commonalities in the visual appearance across a range of visual concepts, thus we clustered to create surrogate labels.
%
    \item For clustering, we use k-means with a fixed k for the entire process of refining. 
    \item The hope is to capture visual semantics, as images that have visual similarity get together in a cluster.
    \item Dimensionality reduction techniques like PCA (retaining $95\%$ variance) have also been tried on the visual features before grouping them with the help of K-means.
\end{itemize}
% * <vrama91@vt.edu> 2015-10-21T09:18:36.411Z:
%
% > Dimensionality reduction techniques like PCA (retaining $95\%$ variance) have also been tried on the visual features before grouping them with the help of K-means.
% > \end{itemize}
%
% Feels more of an experimental detail. We could move it there where we talk about how many "k" in k-means, PCA vs not, etc. We will lay out the set of baseline visual w2v models there. Makes sense?
%
% ^ <satwik27@gmail.com> 2015-10-21T14:52:26.397Z:
%
% Yup, makes sense.
%
% ^.
\subsection{Visual Word2Vec Model}
% * <vrama91@vt.edu> 2015-10-21T09:19:36.167Z:
%
% > Visual Word2Vec Model
%
% Move this above Image Clustering subsection
%
% ^ <satwik27@gmail.com> 2015-10-21T14:53:13.850Z:
%
% Well, if I think of it, that makes sense too.
%
% ^.
\begin{itemize}
	\item Neural network used to train visual word2vec resembles the skip-gram model of word2vec (refer figure). 
% * <vrama91@vt.edu> 2015-10-21T09:20:06.004Z:
%
% > skip-gram
%
% CBOW?
%
% ^ <satwik27@gmail.com> 2015-10-21T14:53:41.693Z:
%
% Lets not draw comparisons then. We just show what our model is like.
%
% ^.
    \item the network has three layer - input, hidden and an output layer.
    \item Following word2vec, we use one-hot encoding at the input layer
% * <vrama91@vt.edu> 2015-10-21T09:22:48.857Z:
%
% >  Following word2vec, we use one-hot encoding at the input layer
%
% Need to describe the word2vec architecture first briefly, then mention how we change it. Will make the subsequent explanation more succinct.
%
% ^ <satwik27@gmail.com> 2015-10-21T14:53:57.569Z:
%
% Done.
%
% ^.
    \item Therefore a vocabulary of size $N_v$ will result in $N_V$ input nodes shown in red in Fig x.
    \item the number of nodes (shown in some color) in the hidden layer $N_H$ is retained as in, from the pre-trained word2vec model.
    \item Although $N_H$ is a design parameter, we stress that our approach cannot be used to change the number of hidden layers compared to pre-trained model.
% * <vrama91@vt.edu> 2015-10-21T09:20:33.617Z:
%
% > tem Although $N_H$ is a design parameter, we stress that our approach cannot be used to change the number of hidden layers compared to pre-trained model.
%
% Since we are finetuning from a text based w2v, we work with the same number of hidden units. In some experiments, we change both and observe its effect. 
%
% ^ <satwik27@gmail.com> 2015-10-21T14:54:37.599Z:
%
% Yup, better as a selling point than a limitation.
%
% ^.
    \item In other words, we have to begin with a word2vec model of appropriate $N_H$.
    \item It is the number of nodes in output layer $N_o$ that visual word2vec and skip-gram model differ.
    \item We remind the readers that we train on the error in predicting the surrogate labels obtained from clustering.
% * <vrama91@vt.edu> 2015-10-21T09:21:37.196Z:
%
% >  clustering.
%
% refer to subsection here
%
% ^ <satwik27@gmail.com> 2015-10-21T14:54:55.747Z:
%
% Yeah, done.
%
% ^.
    \item Similar to the input layer, we use one-hot encoding for these labels.
% * <vrama91@vt.edu> 2015-10-21T09:22:00.093Z:
%
% > m Similar to the input layer, we use one-hot encoding for these labels.
%
% no need tos ay this, just say classification
%
% ^ <satwik27@gmail.com> 2015-10-21T14:55:03.703Z:
%
% Alright
%
% ^.
    \item hence, the number of clusters, k, is a design parameter for the model, resulting in an output layer of size k (shown in some color).
    \item each layer is fully connected to the previous layer, through the corresponding weight matrices: $W_{ih}$ for input to hidden and $W_{ho}$ for hidden to output. $W_{ih}$ is called the inner weight matrix and $w_{ho}$ is called the outer weight matrix.
    \item Representing the output of all the nodes in input layer with $x_i\in \mathbb{R}^N_i$, hidden nodes with $x_h \in \mathbb{R}^N_h$ and output with $x_o \in \mathbb{R}^N_o$, we have: 
    \begin{align}
    	x_h = W_ih  x_i\\
        x_o = w_ho x_h
    \end{align}
    \item Here, $W_ih$ is a $N_V \times N_H$ matrix while $W_ho$ is $N_H \times N_V$. 
    \item explain the rows and columns of these matrices to be the embeddings we are interesting in and show how by using above equations.
% * <vrama91@vt.edu> 2015-10-21T09:23:32.503Z:
%
% > interesting
%
% spell
%
    \hspace{20pt}
    
    \item Given a pre-trained word2vec model, we retain the input and hidden layers. 
    \item However, we discard its output layer along with the outer weight matrix. 
    \item In its place, we have a new output layer with $N_0=N_k$ along with new outer weight matrix $W_ho$. We fill $W_ho$ with random values. 
    \item To summarize, model for visualword2vec is obtained from the pre-trained model by retained the first two layers along with $W_{ih}$, replacing the outer layer with that of size $N_K$ and re-initializing the $W_{ho}$ as a random $N_H \times N_k$ matrix.
    \item Once we construct the visual word2vec model, we begin training it as explained in the following section.
\end{itemize}
    
\subsection{Training}

\begin{itemize}

	\item The objective of the training phase is to refine the weight matrices $W_{ih}$ $W_{ho}$ to learn visually grounded word embeddings.
	\item we do this by back-propagating the loss in predicting the surrogate labels for a given input, from the output to the input layer. 
	\item Consider a training set which is simple pairs of visual feature and associated text i.e  $D = \{(w_1, v_1), (w_2, v_2), ....\}$.
	\item Here, $v_i$ is the visual feature and $W_i$ the text features. $w_i$ could itself be a set of words present in the associated text, $w_i = \{w_{i1}, w_{i2}, ...\}$. For example, $w_i=\{`man', `chases', `dog'\}$.
% * <vrama91@vt.edu> 2015-10-21T09:24:24.414Z:
%
% > Here, $v_i$ is the visual feature and $W_i$ the text features. $w_i$ could itself be a set of words presen
%
% will need to change the tuple format for sentences with VQA
%
% ^ <satwik27@gmail.com> 2015-10-21T14:56:02.404Z:
%
% I did not have the tuple idea in mind when I wrote this. I was meant to be a sentence that got broken down into tokens. Will change the example then.
%
% ^.
	\item By clustering all the visual features (see section), we now have a function $G(.)$ that assigns the cluster id for each visual feature i.e. $G(.)$ maps all the visual features to $\{1, 2, \dots, N_K\}$.
    \item For a given input (bag-of-words) $W_i$, we perform a continuous bag-of-words like prediction where all the weight matrices are assumed to be same. 
% * <vrama91@vt.edu> 2015-10-21T09:24:46.826Z:
%
% > For a given input (bag-of-words) $W_i$, we perform a continuous bag-of-words like prediction where all the weight matrices are assumed to be sam
%
% Its still odd why we take a skip - gram word2vec and then start doing a cbow like thing all of a sudden. Maybe its just best to explain our procedure as it is, without making connections here too much (we have already done this in the intro). What do you think?
%
% ^ <satwik27@gmail.com> 2015-10-21T14:56:33.406Z:
%
% Yup, that avoids unnecessary confusions / conflicts.
%
% ^.
    \item Encoding each word as a one-hot vector, we have:
    \begin{align}
    	x_i &= \frac{1}{|w_i|} {\sum_j{w_{ij}}}\\
        x_h &= w_{ih}x_i\\
        \implies x_h &= \frac{1}{|w_i|} {\sum_j{W_{IH}^{(j)}}}
	\end{align}
    where $W_{IO}^{(j)}$ refers to the $j^{th}$ row of the matrix.
    \item \satwik{write similar equations for final layer and error}
    \item We use multi-class error loss with soft-max.
% * <vrama91@vt.edu> 2015-10-21T09:25:49.485Z:
%
% > write similar equations for final layer and error}
%
% Can go into supplementary
%
% ^ <satwik27@gmail.com> 2015-10-21T14:56:59.871Z:
%
% You mean the equations ? I guess.
%
% ^.
    \item number of clusters is small and we can explicitly compute the denominator for soft-max.
    \item Train the network and update the weights by stochastic gradient descent considering each training instance at a time.
    \item error back propagates through learning rate $\eta$ to outer and inner weight matrices.
    \item we refer the reader to (?) for a detailed derivations of update equations.
    \item \satwik{talk about triplet loss / why we dont use it}
% * <vrama91@vt.edu> 2015-10-21T09:26:22.316Z:
%
% > {talk about triplet loss / why we dont use it}
%
% Move to discussion. Distracting here.
%
% ^ <satwik27@gmail.com> 2015-10-21T14:57:08.944Z:
%
% Cool.
%
% ^.
\end{itemize}
% talk about triplet loss/ why we dont use it 


==> approach/approach_satwik.tex <==

\begin{itemize}
\item different window sizes
\end{itemize}
The two main ingredients to train \vwv{} are: a text corpus, like wikipedia, to train word2vec and a multi-modal collection of visual scenes along with associated text \rama{to refine \wv{} and obtain \vwv{}}.
We refer to the text corpus as base corpus and the multi-modal collection as fine-tuning data.
First, we begin by training word2vec using skip-gram model on the base corpus, as given in ~\cite{Mikolov2013}.
Next, we cluster the features from visual scenes in the fine-tuning data to obtain surrogate labels. 
This clustering is done in the semantically rich abstract scenes feature space.
Finally, by training the model to predict these labels with the associated text as input, we get our \vwv{} embeddings.
We will now describe each of these steps in detail below.

\subsection{\vwv{} Model}
\label{subsec:vis-w2v-model}
As the \vwv{} model is inspired from word2vec, we briefly cover the architecture of word2vec before moving on to \vwv{}.
The word2vec model is a neural network with three layers -- input, hidden, and output layers.
\satwik{For a vocabulary of size $N_V$, words are represented by a one-hot vector where all but one elements are $0$.
The position of the $1$ represents the position of the word in the vocabulary.}
The one-hot encoding of input words results in an input layer with $N_V$ nodes.
The number of nodes in hidden layer $N_H$ is a model design parameter. 
Intuitively, $N_H$ captures the representation power of the model.
The output layer has the same number of nodes as the vocabulary size i.e. $N_V$.
\satwik{Each of these layers are fully connected to the next layer through linear weights with the output layer having an additional softmax non-linearity.}
For example, the output of $i^{th}$ node in input layer is forwarded to the input of $j^{th}$ node in hidden layer with weight $W_{(i, j)}$.
Collecting all these weights, we obtain the inner weight matrix $W$ of size ${N_V\times N_H}$ that connects input layer nodes to the hidden layer.
Similarly, hidden layer nodes are connected to the output layer node through $W'$ of size ${N_H\times K}$, called the outer weight matrix.
Let $x_I \in \mathbb{R}^{N_V}$ denote the output of nodes from input layer, $x_H \in \mathbb{R}^{N_H}$ from the hidden layer, and $x_O \in \mathbb{R}^{N_V}$ from the output layer. 
We have:
\begin{align}
	\label{eq:wordvec-updates}
	x_H &= x_I^T W \\
    x_O &= x_H^T W'
\end{align}
\satwik{With a one-hot input encoding for $x_I$, each word results in $x_H$ being the corresponding row of $W$. For instance, with the $i^{th}$ word in the vocabulary as input, we have $x_H=W^{(i)}$, the $i^{th}$ row of $W$. This gives a $N_H$ length embedding for the $i^{th}$ word.}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.7\columnwidth]{figures/visw2v-model.png}
    \caption{Model for training \vwv{}--input(red), hidden(green) and output(blue) nodes full connected with weight matrices. Input layer has multiple one-hot encoded words predicting the surrogate label of visual scene as a classification problem.}
	\label{fig:vis-w2v-model}
\end{figure}

\satwik{Coming back to \vwv{}, the model is setup to predict the visual context given the corresponding text.
To facilitate this, we allow multiple one-hot encoded input words, each of size $N_V$, all connected to the hidden layer with $W$ of size $N_V \times N_H$.
This accommodates a wide range of textual features for fine-tune data, ranging from scene descriptions to just the primary, secondary object names along with their relation.}
The hidden layer size is retained as $N_H$, from the trained word2vec model.
In order to create surrogate labels, we cluster the visual features (see Sec.~\ref{subsec:clustering}) into $K$ groups (design parameter) and train the \vwv{} as a $K$-way classification problem.
Therefore, the output layer contains $K$ nodes and is connected to the hidden layer through $W'$ of dimensions ${N_H\times K}$.
Fig.~\ref{fig:vis-w2v-model} shows the \vwv{} architecture with the input (red), the hidden (green), and the output nodes (blue).

\satwik{As \vwv{} is initialized from word2vec (see Sec.~\ref{subsec:training}), we describe the construction of \vwv{} model from the latter.
Given the trained word2vec network, we retain the input and hidden layers along with $W$.
The obtained $W$ contains the intermediate embeddings for the words which will be further refined using fine-tune data.}
The output layer, originally of $N_V$ nodes, is replaced with $K$ nodes.
\satwik{The outer weight matrix $W'$ is adjusted to $N_H\times K$ and initialized randomly to begin the second training phase which learns the $W'$ and fine-tunes $W$.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Clustering of images
\subsection{Clustering of Images} \label{subsec:clustering}
\satwik{We remind the reader that we want to learn word embeddings which coherently capture the semantics in both the visual and textual world.
This would require visually similar concepts to belong to the same surrogate class for our training.
To achieve this and to capture the commonalities in the visual appearance across a range of visual concepts, we cluster the visual features of the train data to create the surrogate labels.}
We use k-means to obtain the labels, where $K$ is a model parameter, kept constant throughout training.
Training (Sec.~\ref{subsec:training}) is based on a $K$-way classification of these labels.
\footnote{\satwik{Alternatively, one could regress on the feature values themselves. However, our experiments showed clustering to have superior results.}}
Through this step, the hope is to obtain clusters with high visual similarity within its members.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Training of word2vec
\subsection{Training} \label{subsec:training}
\rama{Although the visual word2vec pipeline itself is task agnostic, we cross validate for the number of clusters}
\satwik{The overall goal is to obtain visually-grounded word embeddings.
We learn the \vwv{} embeddings in two phases.}

\satwik{First, we train word2vec on the base corpus using the skip-gram model as our initialization for multi-modal refining.
In this phase, the model predicts the context around a given input word and trains by minimizing the error.
We choose word2vec as our initialization as it can be trained on huge text corpora.
This is advantageous in two ways: 
i)~The idea of visual-grounding is to learn semantics that are complementary to text using visual scenes. Therefore, such word2vec embeddings capture lot of semantics providing a good starting point.
ii)~It gives us a large coverage in terms of the vocabulary therefore generalizing well to vivid scene descriptions for refining.}
We refer the reader to ~\cite{Mikolov2013} for details on training word2vec.

Next, we obtain the \vwv{} model as elaborated towards the end of Sec.~\ref{subsec:vis-w2v-model} from this word2vec initialization.
For a given textual input (scene descriptions, for instance), the model minimizes the error in predicting the corresponding surrogate label for the visual features.
We update the weight matrices $W$ and $W'$ by backpropagating the classification loss from the output layer back to the input layer, iterating over the fine-tune dataset.

Formally, consider a multi-modal training set, \textit{i.e.},  as a set of pairs of visual scenes and associated text i.e. $D = \{(v_i, w_i)\}_i$.
Here, $v_i$ represents the visual features extracted from the scenes and $w_i$ is the associated text features.
Our \vwv{} model allows a wide range of textual features.
For example, $w_i$ could be a description of the visual scene spanning multiple sentences or just a tuple describing the primary, secondary objects of interest along with their relation.
During training, we pre-process the text by lemmatizing the tokens obtained from the sentences.
Therefore, each of the $w_i$ is a set of words in itself.
Clustering the visual features gives us a grouping function $G(v_i)$ that assigns surrogate labels to each $v_i$, \textit{i.e.}, $G$ maps all the visual features to one of $K$ class labels $\{1,2,\cdots,K\}$.
At each step in training, we select a subset $S_{w_i} \subseteq w_i$ to fine-tune the model.
Encoding each word as one-hot vector of size $N_V$, the input $x_I$ can be written as :
\begin{align}
	\label{eq:model-input}
	x_I &= \frac{1}{|S_{w_i}|} {\sum_{w \in S_{w_i} \subseteq w_i}{w}}
\end{align}

\satwik{If $S_{w_i} = w_i$, fine-tuning of \vwv{} considers the entire text at once. Other choices are: refining with each word at once by taking a singleton $S_{w_i}$, sliding window of words, etc.}
We use the multi-class loss with softmax function to backpropagate the error using stochastic gradient descent.
At each iteration, we pick a training instance $(v_i, w_i)$ and compute the error in predicting $G(v_i)$ when input $x_I$ is as shown in Eq.~\ref{eq:model-input}. From Eq.~\ref{eq:wordvec-updates}:
\begin{align}
	x_H &= x_I^T W' \\
    \implies x_H &= \frac{1}{|S_{W_i}|} {\sum_{w \in S_{w_i} \subseteq w_i} {W^{(w)}}}	
\end{align}
	
At each training epoch, we cycle through the multi-modal data until a suitable stopping criterion is met or iterations exhaust.
Note that as the number of clusters is usually small, \textit{i.e.} K $<<$ V , softmax function can be explicitly computed for the backpropagation update equations.

==> results/results_internal.tex <==
\begin{itemize}
\item how many real have common sense of 1 abstract scene?
\item Results on real image experiment.
\end{itemize}
We first discuss our results and design choices when we learn a \vwv on common sense and test on common sense. We then discuss our results on learning a \vwv on the visual paraphrasing task. We then show some qualitative results to visualize what our embedding has learnt. \rama{For the final version of the paper, we will (hopefully) have results on two other tasks: common sense assertion paraphrasing, common-sense image retrieval based on tuples/assertions, common-sense image clustering, improvements on CIDEr.}
% Table with common sense key results
\begin{table} \footnotesize
\setlength{\tabcolsep}{5.5pt}
\begin{center}
\begin{tabular}{@{} l  c  c @{}}
%\hline
\toprule
Approach & common sense mAP (\%)\\
\midrule
\texttt{$w2v_{coco}$}~\cite{vedantamLICCV15}  &   72.3\\
\texttt{$w2v_{coco}$} + vision~\cite{vedantamLICCV15} & 73.6\\
\texttt{$vis-w2v_{coco}$} (multi) & \textbf{75.2}\\ 
\texttt{$vis-w2v_{coco}$} (single) & 74.2\\
\texttt{$vis-w2v_{coco}$}(ours)+ vision~\cite{vedantamLICCV15} & \textbf{75.2}\\
\bottomrule
%Human & & & & & & & \\
%\hline
\end{tabular}
\caption{Performance of models on the common sense task of ~\cite{vedantamLICCV15}}
\label{table:1}
\vspace{-8pt}
\end{center}
\end{table}

\subsection{Common Sense Results}
We learn \vwv as described in Section.~\ref{sec:4} on the common sense task. As described previously, we investigate two models: multi, which is trained separately for primary, secondary objects and relations, and single, which shares parameters across primary, secondary and relation words. We find that our \vwv-multi model achieves a mean AP of 75.2\% which is a gain of 2.9\% mean AP over the text-based model of ~\cite{vedantamLICCV15} (Table.~\ref{table:1}). Interestingly, our \vwv based text model outperforms the joint text-based model of ~\cite{vedantamLICCV15} by 1.2\% mean AP. The common sense task requires rich reasoning about relation similarity to judge the plausibility of assertions. Thus, these results indicate that our text only model seems to have captured the nuances of relations better than the joint text~+~vision model of ~\cite{vedantamLICCV15}. We also learn their joint text~+~vision model using our \vwv embeddings instead of $w2v_{coco}$ used by them. We find that the joint model does not give any gains over just \vwv. Thus, our model seems to have captured most of the complimentary information present in the visual signals for the common sense task. 

We also invesitgate other design choices such as the dimensionality of the hidden state in \vwv and the number of clusters used for training in the supplementary material. Our best model (with 50 hidden states, 25 clusters) produces an accuracy of 75.4\% on the common sense task. We also found that lower capacity w2v models with smaller hidden states got a greater boost with \vwv than higher capcity models with higher number of hidden states.

\paragraph{Qualitative Results} We visualize the difference in the embeddings learnt by $w2v_{wiki}$ as compared to $vis-w2v_{wiki}$ using t-SNE~\cite{add}. We find \rama{add some interesting examples of which words changed a lot etc. here}

\subsection{Visual Paraphrasing Results}
On the visual paraphrasing task, our model gets around 1\% improvement to 95.1\% over the baseline text model. \rama{We will invesitgate the results in more depth for the submission version, have qualitative results of failures and success cases}
\subsection{Other Qualitative Results}
\rama{In this section, we will probe into what makes the \vwv system tick. We will look at visualizations of the original clusters, analyze which relations (from common sense) co-occur the most, etc. and understand the source of our performance}

\subsection{Other Results}
\rama{As described earlier, we hope to have other results on assertion-based image retrieval, visual paraphrasing on tuple data, improving cider etc. So lots to look forward to!}

\begin{comment}
% Testing some features : remove if in the way
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/single-model-iccv}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/single-multi-iccv}
    \end{subfigure}
    \caption{}
\end{figure*}

\begin{itemize}
\item Interestinly, we never optimize for the common sense task. We dont use their validation set at all.
\end{itemize}
Performance on Common Sense
\begin{itemize}
\item Numbers, ours vs iccv
\item Qualitative examples of wikipedia embeddings vs common sense embeddings
\item Clusters: Which relations co-occur in the same clusters the most? Some figure showing this.
\item Performance with different number of hidden units.
\item Performance with regression to features
\item A nice side experiment: Get CNN features on Clipart scenes. Cluster using CNN features. Do CNN features help visual word2vec more than semantic features?
\end{itemize}
Performance on Visual Paraphrasing

Interestingly, we never optimize to do well on their task, except for hyperparameter tuning.
\begin{itemize}
\item Numbers w2v vs vis-w2v
\item Us vs Xiao's approach 
\item Anything else that is interesting?
\end{itemize}
\end{comment}
